PokeRRT: A Kinodynamic Planning Approach for Poking Manipulation

This work introduces PokeRRT, a novel motion planning algorithm that demonstrates poking as an effective non-prehensile manipulation skill to enable fast manipulation of objects and increase the size of a robot's reachable workspace. Our qualitative and quantitative results demonstrate the advantages of poking over pushing and grasping in planning object trajectories through uncluttered and cluttered environments.

==> table-sim-actions.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
                                                                                     & \multicolumn{6}{c|}{\textbf{Number of Actions in Execution Path}}                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{Planner}}                                               & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S4} & \textbf{S5} & \textbf{S6} \\ \hline
\multicolumn{1}{|c|}{PokeRRT*}                                                       & 
\textbf{\begin{tabular}[c]{@{}c@{}}3.93\\ (0.98)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}4.62\\ (1.04)\end{tabular}}                       
&   \textbf{\begin{tabular}[c]{@{}c@{}}4.49\\ (1.02)\end{tabular}}   
&   \textbf{\begin{tabular}[c]{@{}c@{}}4.76\\ (1.20)\end{tabular}}   
& \textbf{\begin{tabular}[c]{@{}c@{}}3.71\\ (1.02)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}3.65\\ (1.08)\end{tabular}}\\ \hline
\multicolumn{1}{|c|}{PokeRRT} &
  \begin{tabular}[c]{@{}c@{}}6.10 \\ (1.96)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}8.21\\ (2.95)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}7.94\\ (2.08)\end{tabular}  &\begin{tabular}[c]{@{}c@{}}6.77\\ (2.35)\end{tabular}
  &
\begin{tabular}[c]{@{}c@{}}4.56\\ (1.27)\end{tabular}  &
 \begin{tabular}[c]{@{}c@{}}8.17\\ (2.46)\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT*\end{tabular}} & 
\begin{tabular}[c]{@{}c@{}}16.43\\ (2.28)\end{tabular}&
\begin{tabular}[c]{@{}c@{}}22.27\\ (2.26)\end{tabular}
&\begin{tabular}[c]{@{}c@{}}19.00\\ (1.54)\end{tabular}
&\begin{tabular}[c]{@{}c@{}}18.54\\ (1.44)\end{tabular}
&N/A
& N/A            \\ \hline

\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT\end{tabular}} &
\begin{tabular}[c]{@{}c@{}}19.08 \\ (1.51)\end{tabular}
  &
\begin{tabular}[c]{@{}c@{}}19.62\\ (1.64)\end{tabular}  &
 \begin{tabular}[c]{@{}c@{}}20.74\\ (2.13)\end{tabular} &\begin{tabular}[c]{@{}c@{}}19.38\\ (1.59)\end{tabular}
  &
N/A  &
N/A  \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Two-Level\\ Push Planner\end{tabular}} &
\begin{tabular}[c]{@{}c@{}}8.72 \\ (1.42)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}8.61\\ (1.71)\end{tabular}   &
\begin{tabular}[c]{@{}c@{}}7.68\\ (1.19)\end{tabular}   &\begin{tabular}[c]{@{}c@{}}8.53 \\ (1.51)\end{tabular}
  &N/A
   &N/A
   \\ \hline\hline
\multicolumn{1}{|c|}{Pick-and-Place}                                                 & \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}           & N/A           & \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}           & N/A           \\ \hline
\end{tabular}
}
\caption{Number of executed actions in planned path for various planning algorithms in simulation across multiple scenarios. Both \textsl{PokeRRT*} and  \textsl{Low-Impulse PokeRRT*} lead to fewer actions than their respective RRT-based counterparts due to the online path smoothing approach inherent to RRT*.\vspace{-20pt}}
\label{tab:eval-sim-actions}
\end{table}

==> table-sim-rate.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
 &
  \multicolumn{6}{c|}{\textbf{Success Rate}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Planner}} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} \\ \hline
\multicolumn{1}{|c|}{PokeRRT*} &
   \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}0.84\\ (0.37)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}0.73\\ (0.44)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}0.99\\(0.08)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.52\\(0.50)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.88\\(0.33)\end{tabular}
   \\ \hline
\multicolumn{1}{|c|}{PokeRRT} &
  \begin{tabular}[c]{@{}c@{}}0.98\\ (0.13)\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}0.90\\ (0.30)\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}0.76\\ (0.43)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.99\\ (0.09)\end{tabular}
  &\begin{tabular}[c]{@{}c@{}}0.54\\(0.50)\end{tabular}
  &\begin{tabular}[c]{@{}c@{}}0.68\\ (0.47)\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT*\end{tabular}}
   &\begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.47\\ (0.50)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.74\\ (0.44)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.98\\ (0.14)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.00\\(0.00)\end{tabular}
   \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT\end{tabular}} &
\begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}0.86\\ (0.34)\end{tabular}  &
\begin{tabular}[c]{@{}c@{}}0.90\\ (0.29)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular}
  &\begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular}
  &
 \begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Two-Level\\ Push Planner\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}0.52\\ (0.50)\end{tabular}   &
\begin{tabular}[c]{@{}c@{}}0.16\\ (0.37)\end{tabular}   &\begin{tabular}[c]{@{}c@{}}0.97\\ (0.17)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular}
   &\begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular}
   \\ \hline\hline
\multicolumn{1}{|c|}{Pick-and-Place} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular} \\ \hline
\end{tabular}
\caption{asdf}
\label{tab:eval-sim-rate}
\end{table*}

==> table-sim.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-19}
 &
  \multicolumn{6}{c|}{\textbf{Task Time}} &
  \multicolumn{6}{c|}{\textbf{Success Rate}} &
  \multicolumn{6}{c|}{\textbf{Num Actions in Plan}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Planner}} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} \\ \hline
\multicolumn{1}{|c|}{PokeRRT*} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT*\end{tabular}} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \hline
\multicolumn{1}{|c|}{PokeRRT} &
  \begin{tabular}[c]{@{}c@{}}43.06\\ (17.93)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}76.72\\ (26.19)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}0.98\\ (0.14)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}0.95\\ (0.21)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}7.84\\ (2.34)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}12.90\\ (3.84)\end{tabular} &
   &
   \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}97.74\\ (24.72)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}75.32\\ (18.32)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}0.98\\ (0.13)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}25.26\\ (4.95)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}16.97\\ (2.02)\end{tabular} &
   &
   \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Two-Level\\ Push Planner\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}84.14\\ (25.00)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}77.58\\ (26.63)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}0.96\\ (0.19)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}0.99\\ (0.09)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}9.55\\ (2.01)\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}c@{}}9.51\\ (2.24)\end{tabular} &
   &
   \\ \hline
\multicolumn{1}{|c|}{Pick-and-Place} &
  \begin{tabular}[c]{@{}c@{}}16.29\\ (3.76)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}17.71\\ (3.81)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}16.14\\ (3.25)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}240.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}19.15\\ (4.99)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}240.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.00\\ (0.00)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.00\\ (0.00)\end{tabular} &
  - &
  - &
  - &
  - &
  - &
  - \\ \hline
\end{tabular}
\caption{Sim task time = planning time + execution time + replanning time; 250 trials}
\label{tab:eval-sim}
\end{table*}

==> table-success-rate-sim.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Planner} &
  \textbf{Model} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} \\ \hline
\multirow{2}{*}{PokeRRT*} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT*\end{tabular}} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Two-Level\\ Push Planner\end{tabular}} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{Pick-and-Place} &
  - &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\end{tabular}
\caption{Sim success rate}
\label{tab:success-rate-sim}
\end{table}

==> table-task-time-sim.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Planner} &
  \textbf{Model} &
  \textbf{S1} &
  \textbf{S2} &
  \textbf{S3} &
  \textbf{S4} &
  \textbf{S5} &
  \textbf{S6} \\ \hline
\multirow{2}{*}{PokeRRT*} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Low-Impulse\\ PokeRRT*\end{tabular}} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Two-Level\\ Push Planner\end{tabular}} &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \cline{2-8} 
 &
  Learning &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\multirow{2}{*}{Pick-and-Place} &
  - &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0\\ (0)\end{tabular} \\ \hline
\end{tabular}
\caption{Sim task time = planning time + execution time + replanning time}
\label{tab:task-time-sim}
\end{table}
